How to Protect Copyright Data in Optimization of Large Language Models?

Large language models (LLMs) and generative AI have played a transformative role in computer research and applications. Controversy has arisen as to whether these models output copyrighted data, which can occur if the data the models are trained on is copyrighted. LLMs are built on the transformer neural network architecture, which in turn relies on a mathematical computation called Attention that uses the softmax function. In this paper, we show that large language model training and optimization can be seen as a softmax regression problem. We then establish a method of efficiently performing softmax regression, in a way that prevents the regression function from generating copyright data. This establishes a theoretical method of training large language models in a way that avoids generating copyright data.

==> trash/discussion.tex <==
\section{discussion}

Given $Q,K,V \in \R^{n \times d}$
\begin{align*}
D^{-1} \exp(Q K^\top) V
\end{align*}
where $D = \diag( \exp(QK^\top) {\bf 1}_n ) $.


$X_{\ell} \in \R^{n \times d}$

$Q,K,V \in \R^{d \times d}$ weights
\begin{align*}
X_{\ell+1} = \sum_{h=1}^H \underbrace{ D^{-1} }_{n \times n} \underbrace{ \exp(X_{\ell} Q_h K_h^\top X_{\ell}^\top) }_{n \times n} \underbrace{ X_{\ell} }_{n \times d} \underbrace{ V_h }_{d \times d} + X_{\ell} + \mathrm{ReLU}
\end{align*}


One layer, one head, given $X, B$, solve $Q,K,V$
\begin{align*}
f(W,X) = \| D^{-1} \exp(X Q K^\top X) X V - B \|_F^2
\end{align*}

Forward computation $f(W,X)$

Backward computation $\d f(W,X) / \d W$


Let us drop the effect for $XV$, let us target on
\begin{align*}
f(W,X) =  \| D^{-1} \exp(X Q K^\top X) - B \|_F^2
\end{align*}

\Tim{Notes:}
Copyright prevention might be useful at the last layer (fine-tuning process, which happens at last layer) to prevent it from spitting out copyrighted data.

B here represents ground truth (at the last layer). ($X$ is more like $X_{\ell}$, and $B$ is more like $X_{\ell+1}$

Eventually can be applied to multiple layers, but right now apply to the last layer. (Which can motivate why it's a single layer thing.) 

\Tim{Notes on how to write introduction: Follow the Boaz Barak paper. VKB23, is a major copyright theory paper. (They were coming up with some k-anonymity), whereas we are solving it from a different objective function. Their paper is a litlte more about defining copyright data, their paper doesn't quite do it for a network. What kind of loss to add to the last layer, and how to train it.}

VKB23 by boaz is major copyright theory paper.

==> trash/lipschitz.tex <==
\section{Hessian is Lipschitz}\label{sec:lipschitz}


\subsection{Main Result}\label{sec:lipschitz:main_result}

\begin{lemma}[Formal version of Lemma~\ref{lem:lipschitz:informal}]\label{lem:lipschitz}
If the following condition holds
\begin{itemize}
    \item Given two matrices $A_1, A_2 \in \R^{n \times d}$, where $A_1$ is the part of data has copyright
    \item Let $L$ be defined as Definition~\ref{def:L}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    % \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
    \item $H(x) := \frac{\d^2 L}{\d x^2}$
\end{itemize}
Then, we have
\begin{itemize}
    \item 
    \begin{align*}
        \| H(x) - H(y) \| \leq 10000 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2
    \end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
    \begin{align*}
        & ~ \| H(x) - H(y) \| \\
        = & ~ \| ( H_1(x) + H_2(x) + H_3(x) ) - ( H_1(y) + H_2(y) + H_3(y) ) \| \\
        \leq & ~ \| H_1(x) - H_1(y) \| + \| H_2(x) - H_2(y) \| + \| H_3(x) - H_3(y) \| \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2 + \| H_2(x) - H_2(y) \| + \| H_3(x) - H_3(y) \| \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2 + \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 + \| H_3(x) - H_3(y) \| \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2 + \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 + \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2 + 2\beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2 + 2 \gamma^{-4} \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2 + 2 \gamma^{-4} \beta^{-2} n^{1.5}\exp(40R^2)\|x - y\|_2 \\
        \leq & ~ 10000 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2
    \end{align*}
    where the 1st step follows from Lemma~\ref{lem:Hessian_L}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound}, the 3rd step follows from Lemma~\ref{lem:H1_lipschitz}, the 4th step follows from Lemma~\ref{lem:dls23_lipschitz_bound}, the 5th step follows from Lemma~\ref{lem:B_lipschitz_bound}, the 6th step follows from simple algebra, the 7th step follows from $\gamma \in (0, 1)$, the 8th step follows from $\exp(20R^2) \leq \exp(40R^2)$, the last step follows from simple algebra.
\end{proof}

\subsection{Helpful Lemma}

\begin{lemma}\label{lem:H1_lipschitz}
If the following condition holds
\begin{itemize}
    \item Let $Q(x), Q_1(x), Q_2(x), Q_3(x), Q_4(x), Q_5(x)$ be defined as Definition~\ref{def:Q}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
    \item $Q(x) = 16 ( Q_1(x) - Q_2(x) - Q_3(x) + Q_4(x) ) - Q_5(x)$
    \item Let $H_1(x) := \frac{\d^2 \gamma_c \cdot \ell(x)^{-1}}{\d x^2}$
    \item $\| A \| \leq R$
\end{itemize}
Then, we have
\begin{itemize}
    \item Part 1.
    \begin{align*}
        \| Q(x) - Q(y) \| \leq 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(20R^2) \| x - y \|_2
    \end{align*}
    \item Part 2.
    \begin{align*}
        \| H_1(x) - H_1(y) \| \leq 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2
    \end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align}\label{eq:Q_lipschitz_tool1}
        \| Q(x) - Q(y) \|
        = & ~ \| ( 16 ( Q_1(x) - Q_2(x) - Q_3(x) + Q_4(x) ) - Q_5(x) ) \notag \\
        & ~ - ( 16 ( Q_1(y) - Q_2(y) - Q_3(y) + Q_4(y) ) - Q_5(y) ) \| \notag \\
        \leq & ~ 16 \| Q_1(x) - Q_1(y) \| + 16 \| Q_2(x) - Q_2(y) \| \notag \\
        & ~ + 16 \| Q_3(x) - Q_3(y) \| + 16 \| Q_4(x) - Q_4(y) \| + \| Q_5(x) - Q_5(y) \| ) \notag \\
        \leq & ~ 16 ( \| Q_1(x) - Q_1(y) \| + \| Q_2(x) - Q_2(y) \| \notag \\
        & ~ + \| Q_3(x) - Q_3(y) \| + \| Q_4(x) - Q_4(y) \| + \| Q_5(x) - Q_5(y) \| )
    \end{align}
    where the 1st step follows from the Definition of $Q(x)$, the 2nd step follows from Fact~\ref{fact:vec_norm_bound}, the 3rd step follows from simple algebra.

    Then we combine Lemma~\ref{lem:lipschitz_Q1}, Lemma~\ref{lem:lipschitz_Q2}, Lemma~\ref{lem:lipschitz_Q3}, Lemma~\ref{lem:lipschitz_Q4}, we show that
    \begin{align}\label{eq:Q_lipschitz_tool2}
        & ~ \| Q_1(x) - Q_1(y) \| + \| Q_2(x) - Q_2(y) \|  + \| Q_3(x) - Q_3(y) \| + \| Q_4(x) - Q_4(y) \| \notag \\
        \leq & ~ 68 \gamma^{-4} R_f \| x - y \|_2 + 64 \gamma^{-4} R_f \| x - y \|_2 + 64 \gamma^{-4} R_f \| x - y \|_2 + 132 \gamma^{-4} R_f \| x - y \|_2 \notag \\
        = & ~ 328 \gamma^{-4} R_f \| x - y \|_2 \notag \\
        = & ~ 328 \gamma^{-4} \beta^{-2} n^{1.5} \exp(3R^2) \| x - y \|_2 \notag \\
        \leq & ~ 328 \gamma^{-4} \beta^{-2} n^{1.5} \exp(20R^2) \| x - y \|_2
    \end{align}
    where the 2nd step follows from simple algebra, the 3rd step follows from $R_f = \beta^{-2} n^{1.5} \exp(3R^2)$, the 4th step follows from $\exp(3R^2) \leq \exp(20R^2)$.

    So we have
    \begin{align*}
        \| Q(x) - Q(y) \|
        \leq & ~ 16 ( \| Q_1(x) - Q_1(y) \| + \| Q_2(x) - Q_2(y) \| \\
        & ~ + \| Q_3(x) - Q_3(y) \| + \| Q_4(x) - Q_4(y) \| + \| Q_5(x) - Q_5(y) \| ) \\
        \leq & ~ 16 ( 328 \gamma^{-4} \beta^{-2} n^{1.5} \exp(20R^2) \| x - y \|_2 + \| Q_5(x) - Q_5(y) \| ) \\
        \leq & ~ 16 ( 328 \gamma^{-4} \beta^{-2} n^{1.5} \exp(20R^2) \| x - y \|_2 +  89\gamma^{-3} \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2) \\
        = & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(20R^2) \| x - y \|_2
    \end{align*}
    where the 1st step follows from Eq~\eqref{eq:Q_lipschitz_tool1}, the 2nd step follows from Eq~\eqref{eq:Q_lipschitz_tool2}, the 3rd step follows from Lemma~\ref{lem:lipschitz_Q5}, the 4th step follows from simple algebra.

    \textbf{Proof of Part 2.}
    \begin{align*}
        \| H_1(x) - H_1(y) \|
        = & ~ A^\top \| Q(x) - Q(y) \| A \\
        \leq & ~ \| A \| \cdot \| Q(x) - Q(y) \| \cdot \| A \| \\
        \leq & ~ R^2 \cdot \| Q(x) - Q(y) \| \\
        \leq & ~ R^2 \cdot 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(20R^2) \| x - y \|_2 \\
        \leq & ~ 6672 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2
    \end{align*}
    where the 1st step follows from Definition~\ref{def:Q}, the 2nd step follows from simple algebra, the 3rd step follows from $\| A \| \leq R$, the 4th step follows from Part 1 of Lemma~\ref{lem:H1_lipschitz}, the 5th step follows from simple algebra.
\end{proof}

\begin{lemma}[Lemma 7.1 of \cite{dls23}]\label{lem:dls23_lipschitz_bound}
    If the following condition holds
    \begin{itemize}
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $w \in \R^{n \times d}$
        \item Let $W = \diag(w)$
        \item Let $L_{reg}(x) = \| W Ax \|_2$
        \item Let $H_2(x) = \frac{\d^2 ( L_{reg}(x) + 0.5 \ell_1(x) )}{\d x^2}$
    \end{itemize}
    then we have 
    \begin{align*}
        \| H_2(x) - H_2(y) \| \leq \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2
    \end{align*}
\end{lemma}

\subsection{Definition of matrix functions \texorpdfstring{$Q_i(x)$}{}}
\begin{definition}\label{def:Q}
Given the following 
\begin{itemize}
    \item Let $\ell(x)$ be defined as Definition~\ref{def:ell} 
    \item Let $f(x)$ be defined as Definition~\ref{def:f}
    \item Let $c(x)$ be defined as Definition~\ref{def:c}
    \item Let $B(x)$ be defined as Definition~\ref{def:B}
    \item Let $H_1(x) := \frac{\d^2 \gamma_c \cdot \ell_1(x)^{-1}}{\d x^2}$
\end{itemize}
We define $Q_1(x), Q_2(x), Q_3(x), Q_4(x), Q_5(x) \in \R^{n \times n}$ as follows
\begin{itemize}
    \item $Q_1(x) = \underbrace{ \ell(x)^{-3} }_{\mathrm{scalar}} \cdot \underbrace{ \langle f(x), c(x) \rangle^2 }_{ \mathrm{scalar} } \cdot \underbrace{ f(x) }_{n \times 1} \cdot \underbrace{ f(x)^\top }_{1 \times n}$
    \item $Q_2(x) = \underbrace{ \ell(x)^{-3} }_{ \mathrm{scalar} } \cdot \underbrace{ \langle f(x), c(x) \rangle }_{ \mathrm{scalar} } \cdot \underbrace{ ( f(x) \circ c(x) ) }_{ n \times 1 } \cdot \underbrace{ f(x)^\top }_{1 \times n}$
    \item $Q_3(x) = \underbrace{ \ell(x)^{-3} }_{ \mathrm{scalar} } \cdot \underbrace{ \langle f(x), c(x) \rangle }_{ \mathrm{scalar} } \cdot \underbrace{ f(x) }_{n \times 1} \cdot \underbrace{ ( f(x) \circ c(x) )^\top }_{1 \times n}$ 
    \item $Q_4(x) = \underbrace{ \ell(x)^{-3} }_{ \mathrm{scalar} } \cdot \underbrace{ (f(x) \circ c(x)) }_{n \times 1} \cdot \underbrace{ (f(x) \circ c(x))^\top }_{1 \times n}$
    \item $Q_5 (x) = \underbrace{ \ell(x)^{-2} }_{ \mathrm{scalar} } \cdot \underbrace{ B(x) }_{n \times n}$
\end{itemize}

We define $Q(x) \in \R^{n \times n}$ as follows
\begin{align*}
 Q(x) := 16 ( Q_1(x) - Q_2(x) - Q_3(x) + Q_4(x) ) - Q_5(x)
\end{align*}

Note that $H_1(x) = A^\top Q(x) A$.
\end{definition}
%\Tim{What is $H(x)$? Is it the Hessian of $L_{copyright}(x)$?} \Chiwun{It's the Hessian of $\ell(x)^{-1}$} \Tim{Can you formally define this somewhere?} \Zhao{Thanks for pointing out this, we will work on it.} \Zhao{I think we already fixed this, please check the above definition statement. Thanks a lot}

\subsection{Lipschitz property for matrix function \texorpdfstring{$Q_1(x)$}{}}

\begin{lemma}\label{lem:lipschitz_Q1}
If the following condition holds
\begin{itemize}
    \item Let $Q_1(x)$ be defined as Definition~\ref{def:Q}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
\end{itemize}
Then, we have
\begin{itemize}
    \item 
    \begin{align*}
        \| Q_1(x) - Q_1(y) \| \leq 68 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2
    \end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
%    \textbf{Proof of Part 1.} 
    \begin{align*}
        \| Q_1(x) - Q_1(y) \| = & ~ \| \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 \cdot f(x) f(x)^\top - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 \cdot f(y) f(y)^\top \| \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 | \cdot \| f(x) \|_2 \cdot \| f(x) - f(y) \|_2 \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 | \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \|_2 \\
        & ~ + \| f(x) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \cdot \| f(x) \|_2
    \end{align*}
    where the 1st step follows from Part 1 of Definition~\ref{def:Q}, the 2nd step follows from Part 3 of Lemma~\ref{lem:partializ_bound_tool}.

    We define
    \begin{align*}
        Q_{1, 1}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 | \cdot \| f(x) \|_2 \cdot \| f(x) - f(y) \|_2 \\
        Q_{1, 2}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 | \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \|_2 \\
        Q_{1, 3}(x) := & ~ \| f(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \cdot \| f(y) \|_2
    \end{align*}
    where
    \begin{align*}
        \| Q_1(x) - Q_1(x) \| \leq Q_{1, 1}(x) + Q_{1, 2}(x) + Q_{1, 3}(x)
    \end{align*}
    So we can show that
    \begin{align}\label{eq:Q_1_1}
        Q_{1, 1}(x) = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 | \cdot \| f(x) \|_2 \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 4 \gamma^{-3} \cdot \| f(x) \|_2 \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 4 \gamma^{-3} \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 
    \end{align}
    where the 1st follows from the Definition of $Q_{1, 1}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from $\|f(x)\|_2 \leq 1$, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}.
    \begin{align}\label{eq:Q_1_2}
        Q_{2, 1}(x) = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 | \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \|_2 \notag \\
        \leq & ~ 4 \gamma^{-3} \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \|_2 \notag \\
        \leq & ~ 4 \gamma^{-3} \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 
    \end{align}
    where the 1st follows from the Definition of $Q_{2, 1}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from $\|f(x)\|_2 \leq 1$, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}.
    \begin{align}\label{eq:Q_1_3}
         Q_{1, 3}(x) = & ~ \| f(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \cdot \| f(y) \|_2 \notag \\ 
         \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 \notag \\ 
         \leq & ~ 60 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{1, 3}(x)$, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 2 of Lemma~\ref{lem:scalar_lipschitz_tool_ell_f_c}.

    So we have
    \begin{align*}
        \| Q_1(x) - Q_1(x) \| \leq & ~ Q_{1, 1}(x) + Q_{1, 2}(x) + Q_{1, 3}(x) \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{1, 2}(x) + Q_{1, 3}(x) \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{1, 3}(x) \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 60 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \\
        \leq & ~ 68 \gamma^{-4} R_f \cdot \| x - y \|_2
    \end{align*}
    where the 2nd step follows from Eq.~\eqref{eq:Q_1_1}, the 3rd step follows from Eq.~\eqref{eq:Q_1_2}, the 4th step follows from Eq.~\eqref{eq:Q_1_3}, the 5th step follows from simple algebra.

\end{proof}

\subsection{Lipschitz property for matrix function \texorpdfstring{$Q_2(x)$}{}}
\begin{lemma}\label{lem:lipschitz_Q2}
If the following condition holds
\begin{itemize}
    \item Let $Q_2(x)$ be defined as Definition~\ref{def:Q}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
\end{itemize}
We have
\begin{itemize}
    \item 
    \begin{align*}
        \| Q_2(x) - Q_2(y) \| \leq 64 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align*} 
\end{itemize}
\end{lemma}

\begin{proof}

    \begin{align*}
        \| Q_2(x) - Q_2(y) \| 
        = & ~ \| \ell(x)^{-3} \langle f(x), c(x) \rangle ( f(x) \circ c(x) ) f(x)^\top - \ell(y)^{-3} \langle f(y), c(y) \rangle ( f(y) \circ c(y) ) f(y)^\top \| \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) \|_2 \cdot \| f(x) - f(y) \|_2 \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \|_2 \\
        & ~ + \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \|_2
    \end{align*}
    where the 1st step follows from Part 2 of Definition~\ref{def:Q}, the 2nd step follows from Part 3 of Lemma~\ref{lem:partializ_bound_tool}.

    We define
    \begin{align*}
        Q_{2, 1}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) \|_2 \cdot \| f(x) - f(y) \|_2 \\
        Q_{2, 2}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \|_2 \\
        Q_{2, 3}(x) := & ~ \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \|_2
    \end{align*}
    where
    \begin{align*}
        \| Q_2(x) - Q_2(y) \| \leq Q_{2, 1}(x) + Q_{2, 2}(x) + Q_{2, 3}(x)
    \end{align*}
    So we can show that
    \begin{align}\label{eq:Q_2_1}
        Q_{2, 1}(x) = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) \|_2 \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) \circ c(x) \|_2 \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot 2 \cdot \| f(x) - f(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot 2 \cdot R_f \cdot \| x - y \|_2 \notag \\
        = & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{2, 1}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.
    \begin{align}\label{eq:Q_2_2}
        Q_{2, 2}(x) = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot 3 \cdot R_f \cdot \| x - y \|_2 \notag \\
        = & ~ 6 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{2, 1}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from $\|f(x)\|_2 \leq 1$, the 4th step follows from Part 3 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.
    \begin{align}\label{eq:Q_2_3}
        Q_{2, 3}(x) = & ~ \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \|_2 \notag \\
        \leq & ~ \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \notag \\
        \leq & ~ 2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \notag \\
        \leq & ~ 2 \cdot 27 \gamma^{-4} \cdot R_f \| x - y \|_2 \notag \\
        \leq & ~ 54\gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{2, 3}(x)$, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell_f_c}, the last step follows from simple algebra.

    So we have
    \begin{align*}
        \| Q_2(x) - Q_2(y) \| 
        \leq & ~ Q_{2, 1}(x) + Q_{2, 2}(x) + Q_{2, 3}(x) \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{2, 2}(x) + Q_{2, 3}(x) \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 6 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{2, 3}(x) \\
        \leq & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 6 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 54 \gamma^{-4} \cdot R_f \| x - y \|_2 \\
        \leq & ~ 64 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align*}
    where the 2nd step follows from Eq.~\eqref{eq:Q_2_1}, the 3rd step follows from Eq.~\eqref{eq:Q_2_2}, the 4th step follows from Eq.~\eqref{eq:Q_2_3}, the 5th step follows from simple algebra.

    \end{proof}

\subsection{Lipschitz property for matrix function \texorpdfstring{$Q_3(x)$}{}}

\begin{lemma}\label{lem:lipschitz_Q3}
If the following condition holds
\begin{itemize}
    \item Let $Q_3(x)$ be defined as Definition~\ref{def:Q}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
\end{itemize}
We have
\begin{itemize}
    \item 
    \begin{align*}
        \| Q_3(x) - Q_3(y) \| \leq 64 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align*}
\end{itemize}
\end{lemma}

    \begin{proof}

    \textbf{Proof of Part 3.}
    \begin{align*}
        \| Q_3(x) - Q_3(y) \|
        = & ~ \| \ell(x)^{-3} \langle f(x), c(x) \rangle f(x) ( f(x) \circ c(x) )^\top - \ell(y)^{-3} \langle f(y), c(y) \rangle f(y) ( f(y) \circ c(y) )^\top \| \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \\
        & ~ + \| f(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2 
    \end{align*}
    where the 1st step follows from the Definition of $Q_3(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:partializ_bound_tool}.

    We define
    \begin{align*}
        Q_{3, 1}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \\
        Q_{3, 2}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \\
        Q_{3, 3}(x) := & ~ \| f(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2 
    \end{align*}
    where
    \begin{align*}
        \| Q_3(x) - Q_3(y) \| \leq Q_{3, 1}(x) + Q_{3, 2}(x) + Q_{3, 3}(x)
    \end{align*}
    So we can show that
    \begin{align}\label{eq:Q_3_1}
        Q_{3, 1}(x)
        = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) \|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot 3 R_f \| x - y \|_2 \notag \\
        = & ~ 6 \gamma^{-3} \cdot R_f \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{3, 1}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from $\|f(x)\|_2 \leq 1$, the 4th step follows from Part 3 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.
    \begin{align}\label{eq:Q_3_2}
        Q_{3, 2}(x) 
        = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) - f(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot \| f(x) - f(y) \|_2 \cdot 2 \notag \\
        \leq & ~ 2 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 \cdot 2 \notag \\
        = & ~ 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{3, 2}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.
    \begin{align}\label{eq:Q_3_3}
        Q_{3, 3}(x)
        = & ~ \| f(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot 2 \notag \\
        \leq & ~ 27 \gamma^{-4} \cdot R_f \| x - y \|_2 \cdot 2 \notag \\
        = & ~ 54 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{3, 3}(x)$, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell_f_c}, the last step follows from simple algebra.

    So we have
    \begin{align*}
        \| Q_3(x) - Q_3(y) \| 
        \leq & ~ Q_{3, 1}(x) + Q_{3, 2}(x) + Q_{3, 3}(x) \\
        \leq & ~ 6 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{3, 2}(x) + Q_{3, 3}(x) \\
        \leq & ~ 6 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{3, 3}(x) \\
        \leq & ~ 6 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 4 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 54 \gamma^{-4} \cdot R_f \| x - y \|_2 \\
        \leq & ~ 64 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align*}
    where the 1st step follows from Eq.~\eqref{eq:Q_3_1}, the 2nd step follows from Eq.~\eqref{eq:Q_3_2}, the 3rd step follows from Eq.~\eqref{eq:Q_3_3}, the 4th step follows from simple algebra.

\end{proof}

\subsection{Lipschitz property for matrix function \texorpdfstring{$Q_4(x)$}{}}

\begin{lemma}\label{lem:lipschitz_Q4}
If the following condition holds
\begin{itemize}
    \item Let $Q_4(x)$ be defined as Definition~\ref{def:Q}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
\end{itemize}
We have
\begin{itemize} 
    \item %Part 4.
    \begin{align*}
        \| Q_4(x) - Q_4(y) \| \leq 132 \gamma^{-3} \cdot R_f \| x - y \|_2
    \end{align*} 
\end{itemize}
\end{lemma}

\begin{proof}

    %\textbf{Proof of Part 4.}
    \begin{align*}
        \| Q_4(x) - Q_4(y) \| 
        = & ~ \| \ell(x)^{-3} \langle f(x), c(x) \rangle ( f(x) \circ c(x) ) ( f(x) \circ c(x) )^\top \\ 
        & ~ - \ell(y)^{-2} \langle f(y), c(y) \rangle ( f(y) \circ c(y) ) ( f(y) \circ c(y) )^\top \| \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) \|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \\
        & ~ + \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2
    \end{align*}
    where the 1st step follows from the Definition~\ref{def:Q}, the 2nd step follows from Part 3 of Lemma~\ref{lem:partializ_bound_tool}.

    We define
    \begin{align*}
        Q_{4, 1}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x)\|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \\
        Q_{4, 2}(x) := & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \\
        Q_{4, 3}(x) := & ~ \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2
    \end{align*}
    where
    \begin{align*}
        \| Q_4(x) - Q_4(y) \| \leq Q_{4, 1}(x) + Q_{4, 2}(x) + Q_{4, 3}(x)
    \end{align*}
    So we can show that
    \begin{align}\label{eq:Q_4_1}
        Q_{4, 1}(x) 
        = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x)\|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2\gamma^{-3} \cdot \| f(x) \circ c(x)\|_2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2\gamma^{-3} \cdot 2 \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2\gamma^{-3} \cdot 2 \cdot 3 R_f \cdot \| x - y \|_2 \notag \\
        = & ~ 12\gamma^{-3} \cdot R_f \cdot \| x - y \|_2 
    \end{align}
    where the 1st step follows from the Definition of $Q_{4, 1}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 3 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.
    \begin{align}\label{eq:Q_4_2}
        Q_{4, 2}(x) 
        = & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2\gamma^{-3} \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2\gamma^{-3} \cdot \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \cdot 2 \notag \\
        \leq & ~ 2\gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 \cdot 2 \notag \\
        = & ~ 12\gamma^{-3} \cdot R_f \cdot \| x - y \|_2 
    \end{align}
    where the 1st step follows from the Definition of $Q_{4, 2}(x)$, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 3 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.
    \begin{align}\label{eq:Q_4_3}
        Q_{4, 3}(x) 
        = & ~ \| f(y) \circ c(y) \|_2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot \| f(y) \circ c(y) \|_2 \notag \\
        \leq & ~ 2 \cdot | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot 2 \notag \\
        \leq & ~ 2 \cdot 27 \gamma^{-4} \cdot R_f \| x - y \|_2 \cdot 2 \notag \\
        = & ~ 108 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align}
    where the 1st step follows from the Definition of $Q_{4, 3}(x)$, the 2nd step follows from Part 2 of Lemma~\ref{lem:vec_func_norm_bound}, the 3rd step follows Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell_f_c}, the last step follows from simple algebra.

    So we have
    \begin{align*}
        \| Q_4(x) - Q_4(y) \| 
        \leq & ~ Q_{4, 1}(x) + Q_{4, 2}(x) + Q_{4, 3}(x) \\
        \leq & ~ 12 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + Q_{3, 2}(x) + Q_{3, 3}(x) \\
        \leq & ~ 12 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 12 \gamma^{-2} \cdot R_f \cdot \| x - y \|_2 + Q_{3, 3}(x) \\
        \leq & ~ 12 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 12 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 + 108 \gamma^{-4}  \cdot R_f \| x - y \|_2 \\
        \leq & ~ 132 \gamma^{-4} \cdot R_f \| x - y \|_2
    \end{align*}
    where the 2nd step follows from Eq.~\eqref{eq:Q_4_1}, the 3rd step follows from Eq.~\eqref{eq:Q_4_2}, the 4th step follows from Eq.~\eqref{eq:Q_4_3}, the 5th step follows from simple algebra.

\end{proof}


\subsection{Lipschitz property for matrix function \texorpdfstring{$Q_5(x)$}{}}

\begin{lemma}\label{lem:lipschitz_Q5}
If the following condition holds
\begin{itemize}
    \item Let $Q_5(x)$ be defined as Definition~\ref{def:Q}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
\end{itemize}
We have
\begin{itemize}
    \item %Part 5.
    \begin{align*}
        \| Q_5(x) - Q_5(y) \| \leq 89\gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2
    \end{align*}
\end{itemize}
\end{lemma}

\begin{proof}
    We have
    \begin{align*}
        \| Q_5(x) - Q_5(y) \|
        = & ~ \| \ell(x)^{-2} B(x) - \ell(y)^{-2} B(y) \| \\
        \leq & ~ \| \ell(x)^{-2} B(x) - \ell(x)^{-2} B(y) + \ell(x)^{-2} B(y) - \ell(y)^{-2} B(y) \| \\
        \leq & ~ \| \ell(x)^{-2} B(x) - \ell(x)^{-2} B(y)\| + \| \ell(x)^{-2} B(y) - \ell(y)^{-2} B(y) \| \\
        = & ~ | \ell(x)^{-2} | \cdot \| B(x) - B(y)\| + | \ell(x)^{-2} - \ell(y)^{-2} | \cdot \| B(y) \| \\
        \leq & ~ \gamma^{-2} \cdot \| B(x) - B(y)\| + | \ell(x)^{-2} - \ell(y)^{-2} | \cdot \| B(y) \| \\
        \leq & ~ \gamma^{-2} \cdot \| B(x) - B(y)\| + | \ell(x)^{-2} - \ell(y)^{-2} | \cdot 11 \\
        \leq & ~ \gamma^{-2} \cdot \| B(x) - B(y)\| + 8 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 \cdot 11 \\
        \leq & ~ \gamma^{-2} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 +  8 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 \cdot 11 \\
        \leq & ~ \gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 +  8 \gamma^{-3} \cdot R_f \cdot \| x - y \|_2 \cdot 11 \\
        \leq & ~ \gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 +  8 \gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(3R^2) \cdot \| x - y \|_2 \cdot 11 \\
        \leq & ~ \gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 +  8 \gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(20R^2) \cdot \| x - y \|_2 \cdot 11 \\
        \leq & ~ 89\gamma^{-3} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2 \\
        \leq & ~ 89\gamma^{-4} \cdot \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2
    \end{align*}
    where the 1st step follows from Definition~\ref{def:Q}, the 2nd, 3rd, 4th steps follow from Fact~\ref{fact:mat_norm_bound}, the 5th step follows from $\ell(x) \geq \gamma$, the 6th step follows from Part 1 of Lemma~\ref{lem:mat_func_norm_bounds}, the 7th step follows from Part 2 fo Lemma~\ref{lem:scalar_lipschitz_tool_ell}, the 8th step follows from Lemma~\ref{lem:B_lipschitz_bound}, the 9th step follows from $\gamma \in (0, 1)$, the 10th step follows from $R_f = \beta^{-2} n^{1.5} \exp(3R^2)$, the 11st step follows from $\exp(3R^2) \leq \exp(20R^2)$, the 12nd step follows from simple algebra, the last step follows from $\gamma \in (0, 1)$.
\end{proof}

\begin{lemma}\label{lem:B_lipschitz_bound}
    If the following condition holds
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $w \in \R^{n \times d}$
        \item Let $W = \diag(w)$
        \item Let $L_{reg}(x) = \| W Ax \|_2$
        \item Let $H_2(x) = \frac{\d^2 ( L_{reg}(x) + \ell(x) )}{\d x^2}$
    \end{itemize}
    then we have
    \begin{align*}
        \| B(x) - B(y) \| \leq \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2
    \end{align*}

    \begin{proof}
        We have
        \begin{align*}
            \| H_2(x) - H_2(y) \| 
            = & ~ \| \frac{\d^2 ( L_{reg}(x) + \ell(x) )}{\d x^2} - \frac{\d^2 ( L_{reg}(y) + \ell(y) )}{\d y^2} \| \\
            = & ~ \| \frac{\d^2 L_{reg}(x)}{\d x^2} + \frac{\d^2 \ell(x) }{\d x^2} - \frac{\d^2 L_{reg}(y)}{\d y^2} - \frac{\d^2 \ell(y) }{\d y^2} \| \\
        \end{align*}
        where the 1st step follows from the Definition of $H(x)$, the 2nd step follows from simple differential rule.

        So we have
        \begin{align*}
            \| B(x) - B(y) \|
            \leq & ~ A^\top \cdot \| B(x) - B(y) \| \cdot A \\
            = & ~ \| \frac{\d^2 \ell(x) }{\d x^2} - \frac{\d^2 \ell(y) }{\d y^2} \| \\
            \leq & ~ \| \frac{\d^2 L_{reg}(x)}{\d x^2} + \frac{\d^2 \ell(x) }{\d x^2} - \frac{\d^2 L_{reg}(y)}{\d y^2} - \frac{\d^2 \ell(y) }{\d y^2} \| \\
            = & ~ \| H(x) - H(y) \| \\
            \leq & ~ \beta^{-2} n^{1.5}\exp(20R^2)\|x - y\|_2
        \end{align*}
        where the 1st step follows from simple algebra, the 2nd step follows from Lemma~\ref{lem:rewrite_B}, the 3rd step follows from , the 4th step follows from the Definition of $H(x)$, the 5th step follows from Lemma~\ref{lem:dls23_lipschitz_bound}.
    \end{proof}
\end{lemma}



\section{Lipschitz Tools}

\subsection{Lipschitz Tool: Scalar Function}

\begin{lemma}\label{lem:scalar_lipschitz_tool_ell}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $\gamma \in (0, 1)$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $\ell(x)$ be defined as Definition~\ref{def:ell}
        \item $\ell(x) \geq \gamma$
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1.
        \begin{align*}
            | \ell(x) - \ell(y) | \leq 4 R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 2. Let $p \in \{1, 2, 3\}$, then we have
        \begin{align*}
            | \ell(x)^{-p} - \ell(y)^{-p} | \leq 4p \gamma^{-(1 + p)} \cdot R_f \cdot \|x - y\|_2
        \end{align*}
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        | \ell(x) - \ell(y) |
        = & ~ | \langle c(x), c(x) \rangle - \langle c(y), c(y) \rangle | \\
        = & ~ | \langle c(x) - c(y), c(x) + c(y) \rangle | \\
        \leq & ~ \| c(x) - c(y) \|_2 \cdot \| c(x) + c(y) \|_2 \\
        \leq & ~ (\|c(x)\|_2 + \|c(y)\|_2) \cdot \| c(x) - c(y) \|_2 \\
        \leq & ~ 4 \cdot \| c(x) - c(y) \|_2 \\
        \leq & ~ 4 R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vector}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 3rd step follows from Fact~\ref{fact:vec_norm_bound}, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}, the 5th step follows from Part 2 of Lemma~\ref{lem:vec_lipschitz_tool}.

    \textbf{Proof of Part 2.}
    \begin{align*}
        | \ell(x)^{-p} - \ell(y)^{-p} | 
        = & ~ | \ell(x) - \ell(y) | \cdot | \sum_{i = 0}^{p - 1} \ell(x)^{-p + i}\ell(y)^{-i - 1}| \\
        \leq & ~ | \ell(x) - \ell(y) | \cdot | \sum_{i = 0}^{p - 1} \gamma^{-p + i}\gamma^{-i - 1}| \\
        = & ~ | \ell(x) - \ell(y) | \cdot | \sum_{i = 0}^{p - 1} \gamma^{-p - 1} | \\
        = & ~ | \ell(x) - \ell(y) | \cdot (p - 1 + 1) \cdot \gamma^{-p - 1} \\
        \leq & ~ 4 R_f \cdot \|x - y\|_2 \cdot (p - 1 + 1) \cdot \gamma^{-p - 1} \\
        = & ~ 4p \gamma^{-(1 + p)} \cdot R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from $a^p - b^p = (a-b) ( a^{p-1} + a^{p-2} b + \cdots + a b^{p-2} +  b^{p-1} )$, the 2nd step follows from $\ell(x) \geq \gamma$, the 3rd step follows from simple algebra, the 4th step follows from simple algebra, the 5th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell}, the last step follows from simple algebra.

\end{proof}

\begin{lemma}\label{lem:scalar_lipschitz_tool_f_c}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1.
        \begin{align*}
            | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle |\leq 3 R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 2.
        \begin{align*}
            | \langle f(x), c(x) \rangle^2 - \langle f(y), c(y) \rangle^2 |\leq 12 R_f \cdot \|x - y\|_2
        \end{align*}
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle |
        = & ~ | f(x)^\top c(x) - f(y)^\top c(y) | \\
        \leq & ~ \|f(x)\|_2 \cdot \|c(x) - c(y)\|_2 + \|f(x) - f(y)\|_2 \cdot \|c(x)\|_2 \\
        \leq & ~ \|c(x) - c(y)\|_2 + \|f(x) - f(x)\|_2 \cdot \|c(y)\|_2 \\
        \leq & ~ \|c(x) - c(y)\|_2 + 2 \|f(x)^\top - f(x)^\top\|_2 \\
        \leq & ~ R_f \cdot \|x - y\|_2 + 2 \|f(x)^\top - f(x)^\top\|_2 \\
        \leq & ~ R_f \cdot \|x - y\|_2 + 2 R_f \cdot \|x - y\|_2 \\
        \leq & ~ 3 R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vector}, the 2nd step follows from Part 1 of  Lemma~\ref{lem:partializ_bound_tool}, the 3rd step follows from $\|f(x)\| \leq 1$, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}, the 5th step follows from Part 2 of Lemma~\ref{lem:vec_lipschitz_tool}, the 6th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.

    \textbf{Proof of Part 2.}
    \begin{align*}
        | \langle f(x), c(x) \rangle^2 - \langle f(y), c(y) \rangle^2 |
        \leq & ~ | \langle f(x), c(x) \rangle + \langle f(y), c(y) \rangle | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        \leq & ~ | 2 + 2| \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        \leq & ~ | 2 + 2| \cdot 3 R_f \cdot \|x - y\|_2 \\
        = & ~ 12 R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from simple algebra, the 2nd step follows from Part 2 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_f_c}, the 4th step follows from simple algebra.
\end{proof}

\begin{lemma}\label{lem:scalar_lipschitz_tool_ell_f_c}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $\gamma \in (0, 1)$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
        \item Let $\ell(x)$ be defined as Definition~\ref{def:ell}
        \item $\ell(x) \geq \gamma$
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1.
        \begin{align*}
            | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \leq 27 \gamma^{-4} \cdot R_f \| x - y \|_2
        \end{align*}
        \item Part 2.
        \begin{align*}
            | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \leq 60 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2
        \end{align*}
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \\
        = & ~ | \ell(x)^{-3} | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | + | \ell(x)^{-3} - \ell(y)^{-3} | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | + | \ell(x)^{-3} - \ell(y)^{-3} | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + | \ell(x)^{-3} - \ell(y)^{-3} | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + 12 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + 12 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \cdot 2 \\
        = & ~ ( 3 \gamma^{-3} + 24 \gamma^{-4} ) \cdot R_f \| x - y \|_2  \\
        \leq & ~ 27 \gamma^{-4} \cdot R_f \| x - y \|_2 
    \end{align*}
    where the 1st step follows from Part 4 of Lemma~\ref{lem:partializ_bound_tool}, the 2nd step follows from $\ell(x) \geq \gamma$, the 3rd step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_f_c}, the 4th step follows from Part 2 of Lemma~\ref{lem:scalar_lipschitz_tool_ell}, the 5th step follows from Part 2 of Lemma~\ref{lem:func_bounds}, the 6th step follows from simple algebra, the last step follows from $\gamma \in (0, 1)$.

    \textbf{Proof of Part 2.}
    \begin{align*}
        & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot 2 \\
        \leq & ~ 2 \gamma^{-3} \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot 2 \\
        \leq & ~ 2 \gamma^{-3} \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | +  27 \gamma^{-4} \cdot R_f \| x - y \|_2 \cdot 2 \\
        \leq & ~ 2 \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + 27 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \cdot 2 \\
        = & ~ 60 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 
    \end{align*}
    where the 1st step follows from Part 4 of Lemma~\ref{lem:partializ_bound_tool}, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from $\ell(x) \geq \gamma$, the 4th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell_f_c}, the 5th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_f_c}, the 6th step follows from simple algebra.
\end{proof}

\subsection{Lipschitz Tool: Vector Function}

\begin{lemma}\label{lem:vec_lipschitz_tool}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item $\| A \| \leq R$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1. (see Part 4 of Lemma 7.2 in \cite{dls23})
        \begin{align*}
            \|f(x) - f(y)\|_2 \leq R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 2. (see Part 5 of Lemma 7.2 in \cite{dls23})
        \begin{align*}
            \|c(x) - c(y)\|_2 \leq R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 3.
        \begin{align*}
            \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \leq 3 R_f \cdot \| x - y \|_2
        \end{align*}
        \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 3.}
    \begin{align*}
        \| f(x) \circ c(x) - f(y) \circ c(y) \|_2
        \leq & ~ \| f(x) \|_2 \cdot \| c(x) - c(y) \|_2 + \| f(x) - f(y) \|_2 \cdot \| c(y) \|_2 \\
        \leq & ~ \| c(x) - c(y) \|_2 + \| f(x) - f(y) \|_2 \cdot \| c(y) \|_2 \\
        \leq & ~ \| c(x) - c(y) \|_2 + 2 \cdot \| f(x) - f(y) \|_2 \\
        \leq & ~ R_f \cdot \| x - y \|_2 + 2 \cdot \| f(x) - f(y) \|_2 \\
        \leq & ~ R_f \cdot \| x - y \|_2 + 2 R_f \cdot \| x - y \|_2 \\
        = & ~ 3 R_f \cdot \| x - y \|_2
    \end{align*}
    where the 1st step follows from Part 5 of Lemma~\ref{lem:partializ_bound_tool}, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 2 of Lemma~\ref{lem:vec_lipschitz_tool}, the 5th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}, the 6th step follows from simple algebra.

\end{proof}

\section{Helpful Bounds} 

\begin{lemma}\label{lem:vec_func_norm_bound}
    If the following conditions hold
    \begin{itemize}
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
        \item $\|f(x)\|_2 \leq 1$
    \end{itemize}
    then we have
    \begin{itemize}
        \item Part 1. $\|c(x)\|_2 \leq 2 $
        \item Part 2. $\| f(x) \circ c(x) \|_2 \leq 2$
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        \|c(x)\|_2 
        = & ~ \|f(x) - b\|_2 \\
        \leq & ~ \|f(x)\|_2 + \|b\|_2 \\
        \leq & ~ 1 + \|b\|_2 \\
        \leq & ~ 1 + 1 = 2
    \end{align*}
    where the 1st step follow from Definition~\ref{def:c}, the 2nd step follows Fact~\ref{fact:vec_norm_bound}, the 3rd step follows from $\|f(x)\|_2 \leq 1$, the 4th step follows from $\|b\|_2 \leq 1$.

    \textbf{Proof of Part 2.}
    \begin{align*}
        \| f(x) \circ c(x) \|_2
        \leq & ~ \| f(x) \|_2 \cdot \| c(x) \|_2 \\
        \leq & ~ 1 \cdot \| c(x) \|_2 \\
        \leq & ~ 2
    \end{align*}
    where the 1st steps follow from Fact~\ref{fact:vec_norm_bound}, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}.
\end{proof}

\begin{lemma}\label{lem:func_bounds}
    If the following conditions hold
    \begin{itemize}
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
        \item Let $\ell(x)$ be defined as Definition~\ref{def:ell}
        \item $\|f(x)\|_2 \leq 1$
        \item Let $\gamma \in (0, 1)$
        \item $\ell(x) \geq \gamma$
    \end{itemize}
    then we have
    \begin{itemize}
        \item Part 1. $\ell(x) \leq 4$
        \item Part 2. $0.25 \| b \|_2^2 \leq 0 \leq \langle f(x), c(x) \rangle \leq 2$
        \item Part 3. Let $p, q \in \{1, 2, 3\}$, we have $\ell(x)^{-p} \langle f(x), c(x) \rangle^q \leq 2q\gamma^{-p}$
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        \ell(x)
        = & ~ \langle c(x), c(x) \rangle \\
        \leq & ~ \|c(x)\|_2 \cdot \|c(x)\|_2 \\
        \leq & ~ 2 \times 2 = 4
    \end{align*}
    where the 1st step follow from Definition~\ref{def:ell}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}.

    \textbf{Proof of Part 2.}
    On one hand, we have
    \begin{align*}
        \langle f(x), c(x) \rangle
        \leq & ~ \|f(x)\|_2 \cdot \|c(x)\|_2 \\
        \leq & ~ 1 \cdot \|c(x)\|_2 \\
        \leq & ~ 2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}.

    On the other hand, we have
    \begin{align*}
        \langle f(x), c(x) \rangle
        = & ~ \langle f(x), f(x) - b \rangle \\
        = & ~ \| f(x) \|_2^2 - \langle f(x), b \rangle \\
        = & ~ \| f(x) \|_2^2 - \langle f(x), b \rangle + 0.25 \| b \|_2^2 - 0.25 \| b \|_2^2 \\
        = & ~ \| f(x) - 0.5 b \|_2^2 - 0.25 \| b \|_2^2 \\
        \geq & ~ 0 \geq - 0.25 \| b \|_2^2 
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vec_norm_bound}, the 2nd, 3rd, 4th 5th steps follow from simple algebras.

    \textbf{Proof of Part 3.}
    \begin{align*}
        \ell(x)^{-p} \langle f(x), c(x) \rangle^q 
        \leq & ~ \gamma^{-p} \cdot \langle f(x), c(x) \rangle^q \\
        \leq & ~ 2q \gamma^{-p}
    \end{align*}
    where the 1st step follows from $\ell(x) > \gamma$, the 2nd step follows from Part 2 of Lemma~\ref{lem:func_bounds}.
\end{proof}

\begin{lemma}\label{lem:mat_func_norm_bounds}
    If the following conditions hold
    \begin{itemize}
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $B(x)$ be defined as Definition~\ref{def:B}
        \item $\|f(x)\|_2 \leq 1$
    \end{itemize}
    then we have
    \begin{itemize}
        \item Part 1. $\| B(x) \| \leq 11$
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        \| B(x) \| = & ~ \| \langle 3f(x) - 2b, f(x)\rangle \cdot f(x) f(x)^\top \\
        & ~ + \langle f(x) - b, f(x) \rangle \cdot \diag(f(x)) \\
        & ~ + \diag((2f(x) - b) \circ f(x)) \\
        & ~ + (b \circ f(x)) \cdot f(x)^\top + f(x) \cdot (b \circ f(x))^\top \| \\
        \leq & ~ \| \langle 3f(x) - 2b, f(x)\rangle \cdot f(x) f(x)^\top \| \\
        & ~ + \| \langle f(x) - b, f(x) \rangle \cdot \diag(f(x)) \| \\
        & ~ + \| \diag((2f(x) - b) \circ f(x)) \| \\
        & ~ + \| (b \circ f(x)) \cdot f(x)^\top + f(x) \cdot (b \circ f(x))^\top \|
    \end{align*}
    where the 1st step follows from Lemma~\ref{lem:rewrite_B}.

    For the first term
    \begin{align*}
        \| \langle 3f(x) - 2b, f(x)\rangle \cdot f(x) f(x)^\top \|
        \leq & ~ \| \langle 3f(x) - 2b, f(x)\rangle \| \cdot \| f(x) f(x)^\top \| \\ 
        \leq & ~ \| \langle 3f(x) - 2b, f(x)\rangle \| \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\ 
        \leq & ~ \| 3f(x) - 2b \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\ 
        \leq & ~ ( \| 3f(x) \|_2 + \| 2b \|_2 ) \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~ 3 + \| 2b \|_2 \\
        \leq & ~ 3 + 2 = 5
    \end{align*}
    where the 1st, 2nd steps follow from Fact~\ref{fact:mat_norm_bound}, the 3rd, 4th steps follow from Fact~\ref{fact:vec_norm_bound}, the 5th step follows from $\|f(x)\|_2 \leq 1$, the 6th step follows from $\| b \|_2 \leq 1$, the last step follows from simple algebra.

    For the second term
    \begin{align*}
        \| \langle f(x) - b, f(x) \rangle \cdot \diag(f(x)) \|
        \leq & ~ | \langle f(x) - b, f(x) \rangle | \cdot \| \diag(f(x)) \| \\
        \leq & ~ \| f(x) - b \|_2 \cdot \| f(x) \|_2 \cdot \| \diag(f(x)) \| \\
        \leq & ~ \| f(x) - b \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~ ( \| f(x) \|_2 + \| b \|_2 ) \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~  \| b \|_2 \\
        \leq & ~ 1
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:mat_norm_bound}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 3rd, 4th steps follow from Fact~\ref{fact:vec_norm_bound}, the 5th step follows from $\|f(x)\|_2 \leq 1$, the 6th step follows from $\| b \|_2 \leq 1$.

    For the third term
    \begin{align*}
        \| \diag((2f(x) - b) \circ f(x)) \|
        \leq & ~ \| (2f(x) - b) \circ f(x) \|_2 \\
        \leq & ~ \| 2f(x) - b \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~ ( \| 2f(x) \|_2 + \| b \|_2 ) \cdot \| f(x) \|_2 \\
        \leq & ~ 2 + \| b \|_2 \\
        \leq & ~ 2 + 1 = 3
    \end{align*}
    where the 1st, 2nd, 3rd steps follow from Fact~\ref{fact:vec_norm_bound}, the 4th step follows from $\| f(x) \|_2 \leq 1$, the 5th step follows from $\| b \|_2 = 1$, the last step follows from simple algebra.

    For the fourth term
    \begin{align*}
        \| (b \circ f(x)) \cdot f(x)^\top + f(x) \cdot (b \circ f(x))^\top \|
        \leq & ~ \| (b \circ f(x)) \cdot f(x)^\top \| + \| f(x) \cdot (b \circ f(x))^\top \| \\
        \leq & ~ \| b \circ f(x) \|_2 \cdot \| f(x) \|_2 + \| f(x) \|_2 \cdot \| b \circ f(x) \|_2 \\
        \leq & ~ 2 \| b \circ f(x) \|_2 \\
        \leq & ~ 2 (\|b\|_2 \cdot \|f(x)\|_2) \\
        \leq & ~ 2 (\|b\|_2 \cdot 1 ) \\
        \leq & ~ 2 (1 \cdot 1) \\
        = & ~ 2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vec_norm_bound}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound}, the 3rd step follows from $\| f(x) \|_2 \leq 1$, the 4th step follows from $\| b \|_2 = 1$, the last step follows from simple algebra.

    Then we combine four terms, we have
    \begin{align*}
        \| B(x) \| \leq & ~ 5 + 1 + 3 + 2 = 11
    \end{align*}
    where the last step follows from simple algebra.
\end{proof}


==> trash/lipschitz_tool.tex <==


\section{Lipschitz Tools}

\subsection{Lipschitz Tool: Scalar Function}

\begin{lemma}\label{lem:scalar_lipschitz_tool_ell}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $\gamma \in (0, 1)$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $\ell(x)$ be defined as Definition~\ref{def:ell}
        \item $\ell(x) \geq \gamma$
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1.
        \begin{align*}
            | \ell(x) - \ell(y) | \leq 4 R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 2. Let $p \in \{1, 2, 3\}$, then we have
        \begin{align*}
            | \ell(x)^{-p} - \ell(y)^{-p} | \leq 4p \gamma^{-(1 + p)} \cdot R_f \cdot \|x - y\|_2
        \end{align*}
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        | \ell(x) - \ell(y) |
        = & ~ | \langle c(x), c(x) \rangle - \langle c(y), c(y) \rangle | \\
        = & ~ | \langle c(x) - c(y), c(x) + c(y) \rangle | \\
        \leq & ~ \| c(x) - c(y) \|_2 \cdot \| c(x) + c(y) \|_2 \\
        \leq & ~ (\|c(x)\|_2 + \|c(y)\|_2) \cdot \| c(x) - c(y) \|_2 \\
        \leq & ~ 4 \cdot \| c(x) - c(y) \|_2 \\
        \leq & ~ 4 R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vector}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 3rd step follows from Fact~\ref{fact:vec_norm_bound}, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}, the 5th step follows from Part 2 of Lemma~\ref{lem:vec_lipschitz_tool}.

    \textbf{Proof of Part 2.}
    \begin{align*}
        | \ell(x)^{-p} - \ell(y)^{-p} | 
        = & ~ | \ell(x) - \ell(y) | \cdot | \sum_{i = 0}^{p - 1} \ell(x)^{-p + i}\ell(y)^{-i - 1}| \\
        \leq & ~ | \ell(x) - \ell(y) | \cdot | \sum_{i = 0}^{p - 1} \gamma^{-p + i}\gamma^{-i - 1}| \\
        = & ~ | \ell(x) - \ell(y) | \cdot | \sum_{i = 0}^{p - 1} \gamma^{-p - 1} | \\
        = & ~ | \ell(x) - \ell(y) | \cdot (p - 1 + 1) \cdot \gamma^{-p - 1} \\
        \leq & ~ 4 R_f \cdot \|x - y\|_2 \cdot (p - 1 + 1) \cdot \gamma^{-p - 1} \\
        = & ~ 4p \gamma^{-(1 + p)} \cdot R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from $a^p - b^p = (a-b) ( a^{p-1} + a^{p-2} b + \cdots + a b^{p-2} +  b^{p-1} )$, the 2nd step follows from $\ell(x) \geq \gamma$, the 3rd step follows from simple algebra, the 4th step follows from simple algebra, the 5th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell}, the last step follows from simple algebra.

\end{proof}

\begin{lemma}\label{lem:scalar_lipschitz_tool_f_c}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1.
        \begin{align*}
            | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle |\leq 3 R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 2.
        \begin{align*}
            | \langle f(x), c(x) \rangle^2 - \langle f(y), c(y) \rangle^2 |\leq 12 R_f \cdot \|x - y\|_2
        \end{align*}
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle |
        = & ~ | f(x)^\top c(x) - f(y)^\top c(y) | \\
        \leq & ~ \|f(x)\|_2 \cdot \|c(x) - c(y)\|_2 + \|f(x) - f(y)\|_2 \cdot \|c(x)\|_2 \\
        \leq & ~ \|c(x) - c(y)\|_2 + \|f(x) - f(x)\|_2 \cdot \|c(y)\|_2 \\
        \leq & ~ \|c(x) - c(y)\|_2 + 2 \|f(x)^\top - f(x)^\top\|_2 \\
        \leq & ~ R_f \cdot \|x - y\|_2 + 2 \|f(x)^\top - f(x)^\top\|_2 \\
        \leq & ~ R_f \cdot \|x - y\|_2 + 2 R_f \cdot \|x - y\|_2 \\
        \leq & ~ 3 R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vector}, the 2nd step follows from Part 1 of  Lemma~\ref{lem:partializ_bound_tool}, the 3rd step follows from $\|f(x)\| \leq 1$, the 4th step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}, the 5th step follows from Part 2 of Lemma~\ref{lem:vec_lipschitz_tool}, the 6th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}, the last step follows from simple algebra.

    \textbf{Proof of Part 2.}
    \begin{align*}
        | \langle f(x), c(x) \rangle^2 - \langle f(y), c(y) \rangle^2 |
        \leq & ~ | \langle f(x), c(x) \rangle + \langle f(y), c(y) \rangle | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        \leq & ~ | 2 + 2| \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        \leq & ~ | 2 + 2| \cdot 3 R_f \cdot \|x - y\|_2 \\
        = & ~ 12 R_f \cdot \|x - y\|_2
    \end{align*}
    where the 1st step follows from simple algebra, the 2nd step follows from Part 2 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_f_c}, the 4th step follows from simple algebra.
\end{proof}

\begin{lemma}\label{lem:scalar_lipschitz_tool_ell_f_c}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $\gamma \in (0, 1)$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
        \item Let $\ell(x)$ be defined as Definition~\ref{def:ell}
        \item $\ell(x) \geq \gamma$
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1.
        \begin{align*}
            | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \leq 27 \gamma^{-4} \cdot R_f \| x - y \|_2
        \end{align*}
        \item Part 2.
        \begin{align*}
            | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \leq 60 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2
        \end{align*}
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \\
        = & ~ | \ell(x)^{-3} | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | + | \ell(x)^{-3} - \ell(y)^{-3} | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | + | \ell(x)^{-3} - \ell(y)^{-3} | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + | \ell(x)^{-3} - \ell(y)^{-3} | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + 12 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + 12 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \cdot 2 \\
        = & ~ ( 3 \gamma^{-3} + 24 \gamma^{-4} ) \cdot R_f \| x - y \|_2  \\
        \leq & ~ 27 \gamma^{-4} \cdot R_f \| x - y \|_2 
    \end{align*}
    where the 1st step follows from Part 4 of Lemma~\ref{lem:partializ_bound_tool}, the 2nd step follows from $\ell(x) \geq \gamma$, the 3rd step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_f_c}, the 4th step follows from Part 2 of Lemma~\ref{lem:scalar_lipschitz_tool_ell}, the 5th step follows from Part 2 of Lemma~\ref{lem:func_bounds}, the 6th step follows from simple algebra, the last step follows from $\gamma \in (0, 1)$.

    \textbf{Proof of Part 2.}
    \begin{align*}
        & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle^2 - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle^2 | \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot | \langle f(y), c(y) \rangle | \\
        \leq & ~ | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle | \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | \\
        & ~ + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot 2 \\
        \leq & ~ 2 \gamma^{-3} \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | + | \ell(x)^{-3} \cdot \langle f(x), c(x) \rangle - \ell(y)^{-3} \cdot \langle f(y), c(y) \rangle | \cdot 2 \\
        \leq & ~ 2 \gamma^{-3} \cdot | \langle f(x), c(x) \rangle - \langle f(y), c(y) \rangle | +  27 \gamma^{-4} \cdot R_f \| x - y \|_2 \cdot 2 \\
        \leq & ~ 2 \gamma^{-3} \cdot 3 R_f \cdot \| x - y \|_2 + 27 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 \cdot 2 \\
        = & ~ 60 \gamma^{-4} \cdot R_f \cdot \| x - y \|_2 
    \end{align*}
    where the 1st step follows from Part 4 of Lemma~\ref{lem:partializ_bound_tool}, the 2nd step follows from Part 3 of Lemma~\ref{lem:func_bounds}, the 3rd step follows from $\ell(x) \geq \gamma$, the 4th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_ell_f_c}, the 5th step follows from Part 1 of Lemma~\ref{lem:scalar_lipschitz_tool_f_c}, the 6th step follows from simple algebra.
\end{proof}

\subsection{Lipschitz Tool: Vector Function}

\begin{lemma}\label{lem:vec_lipschitz_tool}
    If the following conditions hold
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $\beta \in (0, 0.1)$
        \item Let $R \geq 4$
        \item Let $x, y \in \R^d$ satisfy $\|A(x - y)\|_\infty < 0.01$
        \item $\| A \| \leq R$
        \item Let $R_f := \beta^{-2} n^{1.5} \exp{3R^2}$ 
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
    \end{itemize}
    We have
    \begin{itemize}
        \item Part 1. (see Part 4 of Lemma 7.2 in \cite{dls23})
        \begin{align*}
            \|f(x) - f(y)\|_2 \leq R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 2. (see Part 5 of Lemma 7.2 in \cite{dls23})
        \begin{align*}
            \|c(x) - c(y)\|_2 \leq R_f \cdot \|x - y\|_2
        \end{align*}
        \item Part 3.
        \begin{align*}
            \| f(x) \circ c(x) - f(y) \circ c(y) \|_2 \leq 3 R_f \cdot \| x - y \|_2
        \end{align*}
        \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 3.}
    \begin{align*}
        \| f(x) \circ c(x) - f(y) \circ c(y) \|_2
        \leq & ~ \| f(x) \|_2 \cdot \| c(x) - c(y) \|_2 + \| f(x) - f(y) \|_2 \cdot \| c(y) \|_2 \\
        \leq & ~ \| c(x) - c(y) \|_2 + \| f(x) - f(y) \|_2 \cdot \| c(y) \|_2 \\
        \leq & ~ \| c(x) - c(y) \|_2 + 2 \cdot \| f(x) - f(y) \|_2 \\
        \leq & ~ R_f \cdot \| x - y \|_2 + 2 \cdot \| f(x) - f(y) \|_2 \\
        \leq & ~ R_f \cdot \| x - y \|_2 + 2 R_f \cdot \| x - y \|_2 \\
        = & ~ 3 R_f \cdot \| x - y \|_2
    \end{align*}
    where the 1st step follows from Part 5 of Lemma~\ref{lem:partializ_bound_tool}, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}, the 4th step follows from Part 2 of Lemma~\ref{lem:vec_lipschitz_tool}, the 5th step follows from Part 1 of Lemma~\ref{lem:vec_lipschitz_tool}, the 6th step follows from simple algebra.

\end{proof}

\section{Helpful Bounds} 

\begin{lemma}\label{lem:vec_func_norm_bound}
    If the following conditions hold
    \begin{itemize}
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
        \item $\|f(x)\|_2 \leq 1$
    \end{itemize}
    then we have
    \begin{itemize}
        \item Part 1. $\|c(x)\|_2 \leq 2 $
        \item Part 2. $\| f(x) \circ c(x) \|_2 \leq 2$
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        \|c(x)\|_2 
        = & ~ \|f(x) - b\|_2 \\
        \leq & ~ \|f(x)\|_2 + \|b\|_2 \\
        \leq & ~ 1 + \|b\|_2 \\
        \leq & ~ 1 + 1 = 2
    \end{align*}
    where the 1st step follow from Definition~\ref{def:c}, the 2nd step follows Fact~\ref{fact:vec_norm_bound}, the 3rd step follows from $\|f(x)\|_2 \leq 1$, the 4th step follows from $\|b\|_2 \leq 1$.

    \textbf{Proof of Part 2.}
    \begin{align*}
        \| f(x) \circ c(x) \|_2
        \leq & ~ \| f(x) \|_2 \cdot \| c(x) \|_2 \\
        \leq & ~ 1 \cdot \| c(x) \|_2 \\
        \leq & ~ 2
    \end{align*}
    where the 1st steps follow from Fact~\ref{fact:vec_norm_bound}, the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}.
\end{proof}

\begin{lemma}\label{lem:func_bounds}
    If the following conditions hold
    \begin{itemize}
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $f(x)$ be defined as Definition~\ref{def:f}
        \item Let $c(x)$ be defined as Definition~\ref{def:c}
        \item Let $\ell(x)$ be defined as Definition~\ref{def:ell}
        \item $\|f(x)\|_2 \leq 1$
        \item Let $\gamma \in (0, 1)$
        \item $\ell(x) \geq \gamma$
    \end{itemize}
    then we have
    \begin{itemize}
        \item Part 1. $\ell(x) \leq 4$
        \item Part 2. $0.25 \| b \|_2^2 \leq 0 \leq \langle f(x), c(x) \rangle \leq 2$
        \item Part 3. Let $p, q \in \{1, 2, 3\}$, we have $\ell(x)^{-p} \langle f(x), c(x) \rangle^q \leq 2q\gamma^{-p}$
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        \ell(x)
        = & ~ \langle c(x), c(x) \rangle \\
        \leq & ~ \|c(x)\|_2 \cdot \|c(x)\|_2 \\
        \leq & ~ 2 \times 2 = 4
    \end{align*}
    where the 1st step follow from Definition~\ref{def:ell}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}.

    \textbf{Proof of Part 2.}
    On one hand, we have
    \begin{align*}
        \langle f(x), c(x) \rangle
        \leq & ~ \|f(x)\|_2 \cdot \|c(x)\|_2 \\
        \leq & ~ 1 \cdot \|c(x)\|_2 \\
        \leq & ~ 2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 2nd step follows from $\|f(x)\|_2 \leq 1$, the 3rd step follows from Part 1 of Lemma~\ref{lem:vec_func_norm_bound}.

    On the other hand, we have
    \begin{align*}
        \langle f(x), c(x) \rangle
        = & ~ \langle f(x), f(x) - b \rangle \\
        = & ~ \| f(x) \|_2^2 - \langle f(x), b \rangle \\
        = & ~ \| f(x) \|_2^2 - \langle f(x), b \rangle + 0.25 \| b \|_2^2 - 0.25 \| b \|_2^2 \\
        = & ~ \| f(x) - 0.5 b \|_2^2 - 0.25 \| b \|_2^2 \\
        \geq & ~ 0 \geq - 0.25 \| b \|_2^2 
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vec_norm_bound}, the 2nd, 3rd, 4th 5th steps follow from simple algebras.

    \textbf{Proof of Part 3.}
    \begin{align*}
        \ell(x)^{-p} \langle f(x), c(x) \rangle^q 
        \leq & ~ \gamma^{-p} \cdot \langle f(x), c(x) \rangle^q \\
        \leq & ~ 2q \gamma^{-p}
    \end{align*}
    where the 1st step follows from $\ell(x) > \gamma$, the 2nd step follows from Part 2 of Lemma~\ref{lem:func_bounds}.
\end{proof}

\begin{lemma}\label{lem:mat_func_norm_bounds}
    If the following conditions hold
    \begin{itemize}
        \item Let $b \in \R^{n}$ satisfy that $\| b \|_1 \leq 1$
        \item Let $B(x)$ be defined as Definition~\ref{def:B}
        \item $\|f(x)\|_2 \leq 1$
    \end{itemize}
    then we have
    \begin{itemize}
        \item Part 1. $\| B(x) \| \leq 11$
    \end{itemize}
\end{lemma}

\begin{proof}
    \textbf{Proof of Part 1.}
    \begin{align*}
        \| B(x) \| = & ~ \| \langle 3f(x) - 2b, f(x)\rangle \cdot f(x) f(x)^\top \\
        & ~ + \langle f(x) - b, f(x) \rangle \cdot \diag(f(x)) \\
        & ~ + \diag((2f(x) - b) \circ f(x)) \\
        & ~ + (b \circ f(x)) \cdot f(x)^\top + f(x) \cdot (b \circ f(x))^\top \| \\
        \leq & ~ \| \langle 3f(x) - 2b, f(x)\rangle \cdot f(x) f(x)^\top \| \\
        & ~ + \| \langle f(x) - b, f(x) \rangle \cdot \diag(f(x)) \| \\
        & ~ + \| \diag((2f(x) - b) \circ f(x)) \| \\
        & ~ + \| (b \circ f(x)) \cdot f(x)^\top + f(x) \cdot (b \circ f(x))^\top \|
    \end{align*}
    where the 1st step follows from Lemma~\ref{lem:rewrite_B}.

    For the first term
    \begin{align*}
        \| \langle 3f(x) - 2b, f(x)\rangle \cdot f(x) f(x)^\top \|
        \leq & ~ \| \langle 3f(x) - 2b, f(x)\rangle \| \cdot \| f(x) f(x)^\top \| \\ 
        \leq & ~ \| \langle 3f(x) - 2b, f(x)\rangle \| \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\ 
        \leq & ~ \| 3f(x) - 2b \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\ 
        \leq & ~ ( \| 3f(x) \|_2 + \| 2b \|_2 ) \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~ 3 + \| 2b \|_2 \\
        \leq & ~ 3 + 2 = 5
    \end{align*}
    where the 1st, 2nd steps follow from Fact~\ref{fact:mat_norm_bound}, the 3rd, 4th steps follow from Fact~\ref{fact:vec_norm_bound}, the 5th step follows from $\|f(x)\|_2 \leq 1$, the 6th step follows from $\| b \|_2 \leq 1$, the last step follows from simple algebra.

    For the second term
    \begin{align*}
        \| \langle f(x) - b, f(x) \rangle \cdot \diag(f(x)) \|
        \leq & ~ | \langle f(x) - b, f(x) \rangle | \cdot \| \diag(f(x)) \| \\
        \leq & ~ \| f(x) - b \|_2 \cdot \| f(x) \|_2 \cdot \| \diag(f(x)) \| \\
        \leq & ~ \| f(x) - b \|_2 \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~ ( \| f(x) \|_2 + \| b \|_2 ) \cdot \| f(x) \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~  \| b \|_2 \\
        \leq & ~ 1
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:mat_norm_bound}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound} (Cauchy-Schwarz inequality), the 3rd, 4th steps follow from Fact~\ref{fact:vec_norm_bound}, the 5th step follows from $\|f(x)\|_2 \leq 1$, the 6th step follows from $\| b \|_2 \leq 1$.

    For the third term
    \begin{align*}
        \| \diag((2f(x) - b) \circ f(x)) \|
        \leq & ~ \| (2f(x) - b) \circ f(x) \|_2 \\
        \leq & ~ \| 2f(x) - b \|_2 \cdot \| f(x) \|_2 \\
        \leq & ~ ( \| 2f(x) \|_2 + \| b \|_2 ) \cdot \| f(x) \|_2 \\
        \leq & ~ 2 + \| b \|_2 \\
        \leq & ~ 2 + 1 = 3
    \end{align*}
    where the 1st, 2nd, 3rd steps follow from Fact~\ref{fact:vec_norm_bound}, the 4th step follows from $\| f(x) \|_2 \leq 1$, the 5th step follows from $\| b \|_2 = 1$, the last step follows from simple algebra.

    For the fourth term
    \begin{align*}
        \| (b \circ f(x)) \cdot f(x)^\top + f(x) \cdot (b \circ f(x))^\top \|
        \leq & ~ \| (b \circ f(x)) \cdot f(x)^\top \| + \| f(x) \cdot (b \circ f(x))^\top \| \\
        \leq & ~ \| b \circ f(x) \|_2 \cdot \| f(x) \|_2 + \| f(x) \|_2 \cdot \| b \circ f(x) \|_2 \\
        \leq & ~ 2 \| b \circ f(x) \|_2 \\
        \leq & ~ 2 (\|b\|_2 \cdot \|f(x)\|_2) \\
        \leq & ~ 2 (\|b\|_2 \cdot 1 ) \\
        \leq & ~ 2 (1 \cdot 1) \\
        = & ~ 2
    \end{align*}
    where the 1st step follows from Fact~\ref{fact:vec_norm_bound}, the 2nd step follows from Fact~\ref{fact:vec_norm_bound}, the 3rd step follows from $\| f(x) \|_2 \leq 1$, the 4th step follows from $\| b \|_2 = 1$, the last step follows from simple algebra.

    Then we combine four terms, we have
    \begin{align*}
        \| B(x) \| \leq & ~ 5 + 1 + 3 + 2 = 11
    \end{align*}
    where the last step follows from simple algebra.
\end{proof}


==> trash/short_lipschitz.tex <==
\section{Hessian is Lipschitz}\label{sec:shor_lipschitz}


\subsection{Main Result}

\begin{lemma}[Informal version of Lemma~\ref{lem:lipschitz:informal}]\label{lem:lipschitz:informal}
If the following condition holds
\begin{itemize}
    \item Given two matrices $A_1, A_2 \in \R^{n \times d}$, where $A_1$ is the part of data has copyright
    \item Let $L$ be defined as Definition~\ref{def:L}
    \item Let $\gamma \in (0,1)$
    \item Let $\beta \in (0, 0.1)$
    \item Let $R \geq 4$
    % \item Let $R_f := \beta^{-2} n^{1.5} \exp(3R^2)$
    \item $\ell(x) \geq \gamma$
    \item $H(x) := \frac{\d^2 L}{\d x^2}$
\end{itemize}
Then, we have

    \begin{align*}
        \| H(x) - H(y) \| \leq 10000 \gamma^{-4} \beta^{-2} n^{1.5} \exp(40R^2) \| x - y \|_2
    \end{align*}
\end{lemma}

==> trash/short_preli.tex <==
\section{Preliminary}\label{sec:short_preli}

In this section, we provide the preliminaries used in our paper. In Section~\ref{subsec:notation} we introduce the notations we use. In Section~\ref{subsec:problem_def} we provide the problem definition that we aim to solve.

\subsection{Notations}\label{subsec:notation}

We denote the $\ell_p$ norm of a vector $x$ by $\| x \|_p$, i.e., $\| x \|_1 := \sum^n_{i=1} | x_i |$, $\| x \|_2 := ( \sum^n_{i=1} x_i^2 )^{1/2}$ and $\| x \|_\infty := \max_{i \in [n]} | x_i |$. For a vector $x \in \R^n$, $\exp(x) \in \R^n$ denotes a vector where $\exp(x_i)$ is $\exp(x_i)$ for all $i \in [n]$. For $n > k$, for any matrix $A \in \R^{n \times k}$, we denote the spectral norm of $A$ by $\| A \|$, i.e., $\| A \| := \sup_{x \in \R^k} \| Ax \|_2 / \| x \|_2$. We use $\sigma_{\min}(A)$ to denote the minimum singular value of $A$. Given two vectors $x, y \in \R^n$, we use $\langle x, y \rangle$ to denote $\sum^n_{i=1} x_i y_i$. Given two vectors $x, y \in \R^n$, we use $x \circ y$ to denote a vector that its i-th entry is $x_i y_i$ for all $i \in [n]$. We use $e_i \in \R^n$ to denote a vector where i-th entry is 1 and all the other entries are 0. Let $x \in \R^n$ be a vector. We define $\diag(x) \in \R^{n \times n}$ as the the diagonal matrix whose diagonal entries are given by $\diag(x)_{i, i} = x_i$ for $i = 1, ..., n$, and all off-diagonal entries are zero. For a symmetric matrix $A \in \R^{n \times n}$, we say $A \succeq 0$ (positive semidefinite (PSD)), if for all $x \in R^n$, we have $x^\top A x \geq 0$. The Taylor Series for $\exp(x)$ is $\exp(x) = \sum^\infty_{i=0} \frac{x^i}{i !}$.

\subsection{Problem Definition}\label{subsec:problem_def}

We first provide the definition of problem below.
\begin{definition}[$\tau$-Copyright-Protected]
Given matrix $A \in \R^{n \times d}$ that $A = \begin{bmatrix}
A_1 \\
A_2
\end{bmatrix}$, where $A_1, A_2 \in \R^{n_2 \times d}$ and $n = n_1 + n_2$. $A_1$ is the data has copyright issue and $A_2$ is the data does not have copyright issue. Also, we are given a vector $b \in \R^n$ with $b = \begin{bmatrix}
b_1 \\
b_2
\end{bmatrix}$
where $b_1, b_2 \in \R^{n_2}$. Denote the train objective $L$. Denote $\tau > 0$ a scalar.

If there is a trained model $f_\theta$ with parameter $\theta$ that satisfies
% \begin{align*}
%     L(f_\theta(A), b) \leq \epsilon
% \end{align*}
% and
\begin{align*}
    L(f_\theta(A_1), b_1) \geq \tau + L(f_\theta(A_2), b_2)
\end{align*}
then we say this model $f_\theta$ is $\tau$-Copyright-Protected.
\end{definition}

During the training process of language models, it is common practice to utilize copyrighted data. This practice does not infringe upon copyright protection laws in many nations. However, there exists a possibility of copyright infringement if generative AI produces samples that are substantially similar to copyrighted data. The ideal language model can learn effectively from all data and its output will not be similar to copyrighted data present in its training set. It is worth noting that due to the Infinite Monkey Theorem, it may be unavoidable for generative AI output to resemble some copyrighted data.

==> trash/trash.tex <==
\iffalse
Suppose we choose some random noise vector $c_1 \in \R^n$, then our plan is to solve this question
\begin{align*}
\min_{x \in \R^d} \| A_1 x - (b_1 + c_1) \|_2^2 + \| A_2 x - b_2 \|_2^2
\end{align*}
\Zhao{The above idea is in fact can write another paper, I think. Let me comment it out}
\fi
% \Tim{Right now we address copyright regression for $f(x)$ = softmax. I think it would be awesome (and much easier than softmax) if we also address it for $f(x) = Ax$, basic linear regression, since linear regression is very fundamental. Is this something we can do?}\Chiwun{I think we can apply copy regression on generative models that their last layers are linear neural networks. Denote the train loss is $\ell(x)$, only when we calculate the gradient for the linear layer, its loss equals to $\ell_1(x) + \ell_2(x) + \alpha \ell_2(x)^{-1}$, where $\alpha$ is hyper-parameter, $\ell_2(x)$ is the loss of data that having copyright issue. But when we calculate the gradients of other layers (such as transformers), the loss equals to $\ell_1(x) + \ell_2(x)$. (We can discuss it in future research)}
